DASH: A Meta-Attack Framework for Synthesizing Effective and Stealthy Adversarial Examples

Numerous techniques have been proposed for generating adversarial examples in white-box settings under strict Lp-norm constraints. However, such norm-bounded examples often fail to align well with human perception, and only a few methods specifically explore perceptually aligned adversarial examples. Moreover, it remains unclear whether insights from Lp-constrained attacks can be effectively leveraged to improve perceptual efficacy. In this paper, we introduce DASH, a fully differentiable meta-attack framework that generates effective and perceptually aligned adversarial examples by strategically composing existing Lp-based attack methods. DASH operates in a multi-stage fashion: at each stage, it aggregates candidate adversarial examples from multiple base attacks using learned, adaptive weights and propagates the result to the next stage. A novel meta-loss function guides this process by jointly minimizing misclassification loss and perceptual distortion, enabling the framework to dynamically modulate the contribution of each base attack throughout the stages. We evaluate DASH on adversarially trained models across CIFAR-10, CIFAR-100, and ImageNet. Despite relying solely on Lp-constrained based methods, DASH significantly outperforms state-of-the-art perceptual attacks such as AdvAD, achieving higher attack success rates (e.g., 20.63% improvement) and superior visual quality, as measured by SSIM, LPIPS, and FID (improvements $\approx$ of 11, 0.015, and 5.7, respectively). Furthermore, DASH generalizes well to unseen defenses, making it a practical and strong baseline for evaluating robustness without requiring handcrafted adaptive attacks for each new defense.

==> tables/cw_variant.tex <==
\begin{table*}[htbp]
\centering
\caption{Effectiveness of \textbf{CW} for different loss functions for the robust CIFAR-100 model -- \cite{cui2024decoupled}.}
\label{tab:cw_variant}
% \resizebox{\textwidth}{!}{%
\renewcommand{\arraystretch}{1}
\small\addtolength{\tabcolsep}{1pt}
\begin{tabular}{cccccccccc}
\toprule 
 \multirow{2}{*}{\textbf{Loss}} & \multicolumn{6}{c}{\textbf{ASR (↑)}} & 
\multirow{2}{*}{\textbf{SSIM (↑)}} & \multirow{2}{*}{\textbf{LPIPS (↓)}} & 
\multirow{2}{*}{\textbf{FID (↓)}} \\
\cmidrule(lr){2-7}
&  Base & JPEG & TVM & Ensemble & NRP & Avg. & & & \\
\midrule
 Original loss (hinge\_loss + \( \ell_2 \)) & 100.00 &	32.32 &	52.05 &	38.57 &	47.66 &	54.12 &	98.46 &	0.0028 &	16.27 \\
\daash~ loss & 100.00 &	87.70 &	96.68 &	78.61 &	57.71 &	84.14 &	94.38 &	0.0153 & 32.49 \\

\bottomrule
\end{tabular}
% }
\end{table*}


==> tables/notations.tex <==
\begin{table}[ht]
    \caption{Notations used in the \daash~framework
    % This table summarizes the key symbols and terms used throughout the paper. It includes notations for the attack functions, loss components, classifier models, attack square indexing, and weighting parameters used to balance adversarial strength and perceptual similarity.
    }
    \label{tab:notations}
    \centering
    \renewcommand{\arraystretch}{1}
\small\addtolength{\tabcolsep}{4pt}
    % \renewcommand{\arraystretch}{1.5}  

    \begin{tabular}{c|c}
        \toprule
        \textbf{Notation} & \textbf{Description} \\
        \hline
        $\boldsymbol{\alpha}$ & Learnable parameters of the attack cells  \\
        \hline
        $a_i(x, y)$ & $i$-th attack applied on image $x$ with label $y$ \\
        \hline
        $\mathcal{A}_j(x, y)$ & $j$-th attack stage \\
        \hline
        $x'$ & Adversarial image generated by attack cell \\
        \hline
        $\mathcal{L}_{\text{total}}$ & Total loss combining TCC and SSIM\\
        \hline
        $\mathcal{L}_{\text{tcc}}$ & True Confidence Class Loss  \\
        % \hline
        % $x'^{\text{R.S.}}, x'^{\text{F.S.}}$ & Adversarial examples under Random Smoothing and Feature Squeezing &  \\
        \hline
        $\mathcal{L}_{\text{ssim}}$ & Structural similarity loss between $x$ and $x'$ \\
        \hline
        $f(\cdot)$ & Classifier model \\
        \hline
        $\lambda_{\text{tcc}}, \lambda_{\text{ssim}}$ & Weighting factors for ASR and SSIM loss \\
        \bottomrule
    \end{tabular}
\end{table}

